Vision-Language-Delta-Action: Learning Compact Deltas as Actionable Transition Interfaces for Robotic Manipulation

Robotic manipulation is not merely observation-to-action generation, but the realization of task-specified state changes in the physical world. Existing vision-language-action (VLA) methods directly learn observation-to-action mappings, imposing a substantial learning burden due to the gap between semantic understanding and action execution. Although world-action models (WAMs) improve control through future prediction, modeling complete future states wastes capacity on static appearance and action-irrelevant changes. We propose Vision-Language-Delta-Action (VLDA), a paradigm that reformulates full future prediction as compact actionable transition modeling. Its core is a compact Delta variable that captures latent world-state changes, serving as an interface between vision-language understanding and action generation. VLDA learns Delta through a unified objective composed of the Local Transition Filter (LT-Filter) and Global Transition Anchor (GT-Anchor). LT-Filter captures task-relevant manipulation-centric changes while suppressing static reconstruction biases. GT-Anchor provides coarse future-level regularization to preserve the overall direction of state changes. Delta-Driven Action Refinement (DDAR) further grounds Delta in the action manifold and injects it as a structured seed to guide action denoising. We implement VLDA within LoongForge, an open-source training framework for large-scale foundation and embodied models, using its modular and distributed infrastructure for unified two-stage optimization. Experiments show that VLDA improves long-horizon consistency, robustness, and generalization, validating actionable Delta as an alternative to direct action prediction and full future-state modeling.

==> Tables/libero.tex <==
\begin{table}[ht]
\centering
\caption{Results on the LIBERO benchmark~\cite{libero}. The last three rows present ablation results.}
\vspace{2pt}
\label{tab:libero_main}
\footnotesize
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|ccccc}
        \toprule
        \textbf{Method} & \textbf{Spatial} & \textbf{Object} & \textbf{Goal} & \textbf{Long} & \textbf{Avg.} \\
        \midrule
        InternVLA-M1~\cite{chen2025internvlam1} & 98.0 & 99.0 & 93.8 & 92.6 & 95.9 \\
        gr00t-N1~\cite{bjorck2025gr00t} & 94.4 & 97.6 & 93.0 & 90.6 & 93.9 \\
        OpenVLA~\cite{openvla} & 84.7 & 88.4 & 79.2 & 53.7 & 76.5 \\
        OpenVLA-OFT~\cite{oft} & 97.6 & 98.4 & 97.9 & 94.5 & 97.1 \\
        Diffusion Policy~\cite{diff} & 78.5 & 87.5 & 73.5 & 64.8 & 76.1 \\
        VLA-Adapter~\cite{wang2025vlaadapter} & 97.8 & 99.2 & 97.2 & 95.0 & 97.3 \\
        UniVLA~\cite{univla} & 95.4 & 98.8 & 93.6 & 94.0 & 95.4 \\
        StarVLA-OFT~\cite{starvla} & 97.8 & 98.6 & 96.2 & 93.8 & 96.6 \\
        CronusVLA~\cite{li2025cronusvla} & 97.3 & 99.6 & 96.9 & 94.0 & 97.0 \\
        $\pi_0$~\cite{pi0} & 96.8 & 98.8 & 95.8 & 85.2 & 94.2 \\
        $\pi_{0.5}$~\cite{pi05} & 98.8 & 98.2 & 98.0 & 92.4 & 96.9 \\
        \midrule

        \textbf{VLDA} & \textbf{99.8} & \textbf{99.6} & \textbf{99.4} & \textbf{95.2} & \textbf{98.5} \\
        ~~~~\textit{w/o Delta-Seeded Action Flow} & 98.2 & 98.4 & 98.6 & 93.6 & 97.2 \\
        ~~~~\textit{w/o Transition Pre-Training} & 98.4 & 98.8 & 98.4 & 93.6 & 97.3 \\
        ~~~~\textit{w/ Full-Future Prediction} & 99.0 & 99.0 & 98.6 & 94.6 & 97.8 \\

        
        \bottomrule
    \end{tabular}%
}
\vspace{-5pt}

\end{table}

